Preserving LLM Capabilities through Calibration Data Curation: From Analysis to Optimization

Post-training compression has been a widely employed approach to scale down large language model (LLM) and facilitate efficient inference. In various proposed compression methods, including pruning and quantization, calibration data plays a vital role by informing the weight importance and activation dynamic ranges. However, how calibration data impacts the LLM capability after compression is less explored. Few of the existing works, though recognizing the significance of this study, only investigate the language modeling or commonsense reasoning performance degradation from limited angles, like the data sources or sample amounts. More systematic research is still needed to examine the impacts on different LLM capabilities in terms of compositional properties and domain correspondence of calibration data. In this work, we aim at bridging this gap and further analyze underlying influencing mechanisms from the activation pattern perspective. Especially, we explore the calibration data's impacts on high-level complex reasoning capabilities, like math problem solving and code generation. Delving into the underlying mechanism, we find that the representativeness and diversity in activation space more fundamentally determine the quality of calibration data. Finally, we propose a calibration data curation framework based on such observations and analysis, enhancing the performance of existing post-training compression methods on preserving critical LLM capabilities. Our code is provided in \href{https://github.com/BokwaiHo/COLA.git}{Link}.

==> curate_original.tex <==
\section{Optimizing Capability Preservation with Calibration Data Curation}
\subsection{Discussion on Calibration Data Optimality for Capability Preservation (Q3)} 
%Some people simply take the `good’ SFT or pre-training data as the `good' calibration data.
%Calibration data is like a ``diagnostic test" that checks all functions. SFT/pre-training data is like a ``textbook" that teaches new knowledge. Good calibration data aims to capture the ``activation pattern" or ``behavioral characteristics" of the model, and focuses on diverse examples that trigger different weight activations. Good SFT/pre-training data aims to teach the model new knowledge/capabilities or adjust its behavior, and focuses on comprehensive coverage of target knowledge/capabilities. Thus, for calibration data, Quality $>$ Quantity: needs clean, diverse cases that exercise different model capabilities. However, for SFT/pre-training data, Quantity + Quality: needs both scale and quality to build robust capabilities.

%Good calibration data for LLM compression is a compact yet diverse set of samples that effectively triggers different activation patterns across model components, covering various tasks and input distributions while being representative of the model's intended use cases. The final goal is to trigger LLM's high-level critical capabilities like reasoning than just telling some fluent nonsense.
Based on our extensive empirical explorations, we can now characterize what constitutes optimal calibration data for preserving LLM capabilities during compression. Our experiments directly revealed the importance of two observable dimensions—compositional properties and domain correspondence—which ultimately point to a deeper mechanistic explanation involving representativeness and diversity in activation space.

\textbf{Compositional Properties}: Our experiments on sequence length, sample amounts, and data sources revealed significant impacts on capability preservation. Longer sequences (2048 tokens) generally provided better performance, though with varying sensitivity across compression methods. Sample amounts showed diminishing returns beyond 64-128 samples, with different saturation points for different methods. Data sources (WikiText, C4, SlimPajama) affected capabilities differently, with no universally optimal source. These findings suggest that optimizing compositional properties forms the foundation of effective calibration.

\textbf{Domain Correspondence}: Our investigations into language, subject, and reasoning difficulty demonstrated that alignment between calibration data and deployment scenarios is crucial. Language-matching calibration data proved especially important for multilingual applications. Subject-aligned calibration data (CommonsenseQA, MathQA, CodeQA) significantly enhanced corresponding capabilities while sacrificing general language modeling. Reasoning difficulty experiments showed mixed difficulty calibration provided the best balance between specialized capabilities and general performance. These findings emphasize that domain correspondence is essential for targeted capability preservation.

\textbf{Underlying Mechanism: Representativeness and Diversity in Activation Space}: Our analyses suggest that the efficacy of compositional properties and domain correspondence stems from a more fundamental mechanism—how calibration data activates the model's parameter space: \textit{Representativeness} in activation space refers to how well calibration samples trigger activation patterns typical of the target deployment domain. This explains why domain-matched calibration data preserved corresponding capabilities so effectively—it activates the specific neural pathways most relevant to the target tasks.
\textit{Diversity} in activation space concerns the breadth of unique activation patterns triggered across the model's parameters. The success of mixed difficulty calibration and format-rich samples (Q\&A w/ ERC) demonstrates that diverse activation patterns enable more comprehensive capability preservation.

The non-monotonic relationships observed in our experiments suggest that selecting samples based on their activation patterns—rather than surface characteristics alone—is the key to optimal calibration.
This mechanistic understanding suggests an approach to calibration data optimization that progresses from observable data characteristics to activation-space considerations. For general-purpose LLM deployment, calibration data should maximize activation diversity while maintaining balanced representation across domains. For specialized applications, calibration data should prioritize representativeness in the target domain's activation patterns while maintaining sufficient diversity to preserve fundamental capabilities.
In light of these findings, we define optimal calibration data for LLM compression as \textbf{a strategically curated set of samples that maximizes both representativeness and diversity in the model's activation space, with the balance determined by deployment requirements.}

\subsection{Calibration Data Curation Framework (Q4)}
\label{sec:framework}
Based on our comprehensive analysis of how calibration data characteristics affect capability preservation and above discussion on calibration data optimality, we propose a three-stage framework for curating optimal calibration data for LLM compression.

\paragraph{Stage 1: Dataset Selection (Domain Correspondence)}
The first stage focuses on selecting source datasets that align with the target deployment domain. This involves analyzing whether the compressed model is intended for general-purpose use or specialized tasks. For general-purpose deployment, we recommend selecting a balanced mix of pre-training datasets (e.g., WikiText for language modeling, SlimPajama for commonsense reasoning, C4 for code generation). For specialized deployment, domain-matched datasets should be prioritized (e.g., MathQA for mathematical problem solving applications). 
Language alignment is crucial in this stage, where datasets in the primary language of intended use should be selected. For multilingual applications, calibration data in each target language should be included, with proportions reflecting deployment priorities. Subject coverage must ensure all critical domains required for deployment are represented.
Reasoning difficulty is also determined at this stage. Based on our experiments, mixed difficulty calibration data provides the best balance for general-purpose deployment, while hard samples may be preferable for specialized reasoning applications. The dataset selection can be formulated as an optimization problem:
\begin{equation}
S = \arg\max_{S \subseteq \mathcal{D}} \sum_{c \in C} w_c \cdot \text{coverage}(S, c)
\label{equ:stage1}
\end{equation}
where $S$ is the selected dataset, $\mathcal{D}$ is the pool of available datasets, $C$ is the set of target capabilities, $w_c$ is the importance weight for capability $c$, and $\text{coverage}(S, c)$ measures how well dataset $S$ covers capability $c$.

\paragraph{Stage 2: Dataset Processing (Compositional Properties)}
The second stage optimizes the compositional properties of the selected datasets. This includes sequence length optimization, where datasets are processed to generate sequences of appropriate length (typically 2048 tokens for most methods, but adaptable based on the specific compression method). For AWQ, which showed robustness to sequence length variation, shorter sequences (512-1024 tokens) may be sufficient.
Format enrichment is another key processing step. For datasets lacking structural richness, we enhance them by converting to Q\&A format with explicit reasoning chains where possible. This involves identifying implicit reasoning in text passages, reformulating as question-answer pairs, and adding intermediate reasoning steps when beneficial.

\paragraph{Stage 3: Sample Selection (Representativeness and Diversity in Activation Space)}
The final stage selects individual samples to maximize representativeness and diversity in activation space. This begins with activation pattern extraction, where for a candidate pool of processed samples, we run a forward pass through the uncompressed model and extract layer-wise activation patterns. For each sample $x_i$, we compute an activation signature vector $\mathbf{a}_i$:
\begin{equation}
\mathbf{a}_i = \left[ \mathbf{h}^1_i, \mathbf{h}^2_i, \ldots, \mathbf{h}^L_i \right]
\end{equation}
where $\mathbf{h}^l_i$ represents the aggregated hidden state activations at layer $l$ for sample $x_i$.
We then apply dimensionality reduction to the activation signatures using Principal Component Analysis (PCA) followed by k-means clustering:
\begin{equation}
\mathbf{a}'_i = \text{PCA}(\mathbf{a}_i, d)
\end{equation}
\begin{equation}
\{C_1, C_2, \ldots, C_k\} = \text{k-means}(\{\mathbf{a}'_1, \mathbf{a}'_2, \ldots, \mathbf{a}'_n\}, k)
\end{equation}
where $d$ is the reduced dimension and $k$ is the target number of clusters.
From each cluster $C_j$, we select samples closest to the centroid to form the final calibration set:
\begin{equation}
x_j^* = \arg\min_{x_i \in C_j} \|\mathbf{a}'_i - \mu_j\|_2
\end{equation}
where $\mu_j$ is the centroid of cluster $C_j$.
Our framework acknowledges that different compression methods require different calibration optimization strategies. For AWQ, which showed remarkable robustness to calibration data variations, a smaller but diverse set of samples may suffice. For pruning methods like SparseGPT, which exhibited higher sensitivity to calibration data characteristics, more careful domain alignment and comprehensive activation pattern coverage are critical.

By systematically addressing dataset-level domain correspondence, compositional characteristics, and ultimately sample-level activation space representation, our curation framework produces compact, high-quality calibration datasets that maximize capability preservation for LLM compression across diverse deployment scenarios.

\begin{table}[h]
\centering
\caption{Performance comparison of different calibration data approaches on general deployment scenario. The best performing approach under each capability is in \textbf{bold}.}
\label{tab:general_deployment}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{4}{c}{LLaMA3-8B} & \multicolumn{4}{c}{Qwen2.5-7B} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& PPL$\downarrow$ & CS$\uparrow$ & Math$\uparrow$ & Code$\uparrow$ & PPL$\downarrow$ & CS$\uparrow$ & Math$\uparrow$ & Code$\uparrow$ \\
\midrule
\multicolumn{9}{c}{\textit{SparseGPT (50\%)}} \\
\midrule
WikiText (random) & 20.15 & 41.85 & 19.18 & 15.34 & 21.54 & 42.23 & 17.85 & 13.45 \\
C4 (random) & 19.36 & 42.67 & 19.64 & 15.88 & 20.85 & 43.12 & 18.24 & 13.87 \\
SlimPajama (random) & 19.58 & 42.81 & 19.78 & 15.77 & 20.98 & 43.29 & 18.37 & 13.80 \\
Self-Gen & 19.65 & 43.61 & 19.85 & 15.92 & 21.07 & 43.92 & 18.42 & 13.92 \\
Ours & \textbf{19.31} & \textbf{44.23} & \textbf{20.12} & \textbf{16.14} & \textbf{20.72} & \textbf{44.47} & \textbf{18.65} & \textbf{14.10} \\
\midrule
\multicolumn{9}{c}{\textit{Wanda (4:8)}} \\
\midrule
WikiText (random) & 33.41 & 40.87 & 18.44 & 14.72 & 32.84 & 40.21 & 17.32 & 12.97 \\
C4 (random) & 32.62 & 41.52 & 18.82 & 15.14 & 32.15 & 40.83 & 17.66 & 13.31 \\
SlimPajama (random) & 32.83 & 41.65 & 18.98 & 15.06 & 32.24 & 40.92 & 17.83 & 13.24 \\
Self-Gen & 32.87 & 42.61 & 19.07 & 15.28 & 32.32 & 41.82 & 17.87 & 13.42 \\
Ours  & \textbf{32.14} & \textbf{43.15} & \textbf{19.36} & \textbf{15.46} & \textbf{31.65} & \textbf{42.34} & \textbf{18.15} & \textbf{13.59} \\
\midrule
\multicolumn{9}{c}{\textit{GPTQ (4-bit)}} \\
\midrule
WikiText (random) & 16.29 & 65.23 & 31.22 & 34.83 & 17.22 & 65.84 & 35.85 & 34.03 \\
C4 (random) & 15.93 & 66.15 & 31.87 & 35.80 & 16.86 & 66.89 & 36.50 & 34.92 \\
SlimPajama (random) & 16.01 & 66.47 & 32.00 & 35.56 & 16.95 & 67.17 & 36.68 & 34.68 \\
Self-Gen & 16.03 & 67.14 & 32.22 & 35.91 & 16.98 & 67.74 & 36.89 & 35.02 \\
Ours  & \textbf{15.83} & \textbf{67.52} & \textbf{32.56} & \textbf{36.18} & \textbf{16.79} & \textbf{68.15} & \textbf{37.23} & \textbf{35.22} \\
\midrule
\multicolumn{9}{c}{\textit{AWQ (4-bit)}} \\
\midrule
WikiText (random) & 15.86 & 65.26 & 36.46 & 38.71 & 17.36 & 66.42 & 47.34 & 62.10 \\
C4 (random) & 15.48 & 66.21 & 37.19 & 39.87 & 17.00 & 67.42 & 48.29 & 63.72 \\
SlimPajama (random) & 15.55 & 66.53 & 37.36 & 39.48 & 17.08 & 67.75 & 48.46 & 63.28 \\
Self-Gen & 15.59 & 67.08 & 37.51 & 39.75 & 17.12 & 68.04 & 48.66 & 63.67 \\
Ours  & \textbf{15.41} & \textbf{67.42} & \textbf{37.85} & \textbf{40.17} & \textbf{16.95} & \textbf{68.47} & \textbf{49.02} & \textbf{64.15} \\
\bottomrule
\end{tabular}%
}
\end{table}

\subsection{Empirical Performance Evaluation}
\paragraph{Framework Implementation}
To evaluate our calibration data curation framework, we conduct comprehensive experiments on LLaMA3-8B-Instruct and Qwen2.5-7B-Instruct. For dataset selection (Stage 1), we implement the coverage function in Equ.~\ref{equ:stage1} as follows:
\begin{equation}
\text{coverage}(S, c) = \alpha \cdot \text{EmbSim}(S, D_c) + (1-\alpha) \cdot \text{KL}(P_S \parallel P_{D_c})
\end{equation}
where $\text{EmbSim}$ is the average cosine similarity between sentence embeddings from both datasets, $\text{KL}$ is the KL-divergence between token distributions, and $\alpha$ is a balancing hyperparameter set to 0.6 in our experiments. This scoring function helps select calibration data sources that best match the target deployment domain in both semantic content and statistical properties. As for $w_c$ in Equ.~\ref{equ:stage1}, for general deployment, we set balanced weights across capabilities, while for specific deployment scenarios, we increase weights for the corresponding target capabilities.
For data processing (Stage 2) and sample selection (Stage 3), we follow the implementation details described in Section~\ref{sec:framework}.  For clustering in the activation space, we run k-means with $k=128$ after dimensionality reduction to 64 components via PCA.

\paragraph{Results and Analysis}
We evaluate our calibration data curation framework across two settings: general deployment and targeted deployment. We compare against random samples from standard pre-training datasets (WikiText, C4, SlimPajama) for general deployment, and random samples from domain-specific datasets for targeted deployment. Besides, we consider the recent Self-Generating then Sampling (Self-Gen) baseline~\citep{ji2024beware}.
\begin{table}[h]
\centering
\caption{Performance comparison of different calibration data approaches for targeted deployment scenarios. The best performing approach under each capability is in \textbf{bold}.}
\label{tab:specific_deployment}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{4}{c}{LLaMA3-8B} & \multicolumn{4}{c}{Qwen2.5-7B} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& PPL$\downarrow$ & CS$\uparrow$ & Math$\uparrow$ & Code$\uparrow$ & PPL$\downarrow$ & CS$\uparrow$ & Math$\uparrow$ & Code$\uparrow$ \\
\midrule
\multicolumn{9}{c}{\textit{Math-focused Deployment (GPTQ 4-bit)}} \\
\midrule
Domain-specific data (random)& 19.87 & 63.21 & 36.92 & 32.18 & 20.14 & 64.36 & 42.36 & 32.41 \\
Self-Gen & 19.65 & 63.84 & 37.65 & 32.78 & 19.96 & 64.98 & 43.17 & 32.95 \\
Ours & \textbf{19.43} & \textbf{64.15} & \textbf{38.92} & \textbf{33.12} & \textbf{19.74} & \textbf{65.42} & \textbf{44.62} & \textbf{33.27} \\
\midrule
\multicolumn{9}{c}{\textit{Code-focused Deployment (GPTQ 4-bit)}} \\
\midrule
Domain-specific data (random) & 19.34 & 62.84 & 29.75 & 39.26 & 19.58 & 63.78 & 32.61 & 42.85 \\
Self-Gen & 19.28 & 63.25 & 30.21 & 40.05 & 19.49 & 64.13 & 33.18 & 43.76 \\
Ours  & \textbf{19.05} & \textbf{63.67} & \textbf{30.64} & \textbf{41.73} & \textbf{19.24} & \textbf{64.52} & \textbf{33.64} & \textbf{45.28} \\
\midrule
\multicolumn{9}{c}{\textit{Multilingual Deployment (GPTQ 4-bit)}} \\
\midrule
Domain-specific data (random)& 18.72 & 64.87 & 30.24 & 33.45 & 18.95 & 65.98 & 34.26 & 33.82 \\
Self-Gen & 18.65 & 65.32 & 30.65 & 33.92 & 18.83 & 66.57 & 34.75 & 34.24 \\
Ours & \textbf{18.41} & \textbf{65.94} & \textbf{31.12} & \textbf{34.26} & \textbf{18.62} & \textbf{67.32} & \textbf{35.21} & \textbf{34.85} \\
\bottomrule
\end{tabular}%
}
\end{table}

For general deployment scenarios (Table \ref{tab:general_deployment}), our activation-aware curation framework consistently outperforms both random sampling and Self-Gen approaches across all capabilities and compression methods. For LLaMA3-8B with SparseGPT, our approach achieves 44.23\% on commonsense reasoning tasks compared to 41.85\% for WikiText random sampling and 43.61\% for the Self-Gen approach. While the absolute improvements appear modest (around 1-2 percentage points), they are consistent across different models, capabilities, and compression methods. The improvements are particularly noticeable for pruning methods (SparseGPT and Wanda), which aligns with our earlier observation that pruning methods exhibit higher sensitivity to calibration data quality.

For targeted deployment scenarios (Table \ref{tab:specific_deployment}), we evaluate three targeted applications: mathematical problem solving, code generation, and multilingual understanding. Our domain-optimized curation framework, which prioritizes representativeness in the target domain while maintaining sufficient diversity, outperforms both random sampling from domain-specific data and Self-Gen approaches. For math-focused deployment on LLaMA3-8B, our approach achieves 38.92\% on mathematical tasks, a 2 percentage point improvement over domain-specific data alone (36.92\%). Similar improvements are observed for code generation (from 39.26\% to 41.73\%) and multilingual scenarios (from 64.87\% to 65.94\% for commonsense reasoning).

The performance gains from our curation framework demonstrate that strategically selecting calibration data based on activation patterns provides significant benefits for capability preservation in compressed LLMs. By optimizing both representativeness and diversity in the activation space, our approach successfully preserve critical capabilities achieves better performance. These results validate our hypothesis that the efficacy of calibration data stems from how it activates the model's parameter space rather than solely from its observable characteristics.

==> explore_original.tex <==
\section{Exploring Calibration Data Variation's Impact on LLM Capabilities}
\subsection{Experiment Preparation}
\paragraph{Large Language Models} We employ the following two powerful and representative open-sourced LLMs to conduct the exploration: LLaMA3-8B-Instruct~\citep{dubey2024llama} and Qwen2.5-7B-Instruct~\citep{yang2024qwen2}. They are both multilingual LLMs, possessing general knowledge and a certain level of reasoning ability.

\paragraph{LLM Compression Schemes} To ensure comprehensiveness, we select two representative post-training pruning methods: SparseGPT~\citep{sparsegpt} for unstructured pruning and Wanda~\citep{wanda} for semi-structured pruning. The pruning ratio is set as 50\% for SparseGPT, and the block pattern is set as $4:8$ for Wanda. We did not conduct experiments with structured pruning methods, considering their performance degradation is super significant under high pruning ratios. As for the post-training quantization, we choose the widely adopted GPTQ~\citep{gptq} and more recent AWQ~\citep{awq} with the bit number set as 4.

\paragraph{Calibration Data Sources} The calibration data can be generally classified into two categories: \textbf{pre-training data} and \textbf{downstream data}. As for the first category, similar to previous works, we take the following datasets as the calibration data sources: \textbf{C4}~\citep{RaffelSRLNMZLL20}, \textbf{WikiText}, and \textbf{SlimPajama}. Except for the experiments investigating the impact of sample amounts and sequence lengths, we randomly sample 128 sequences with the token length as 2048 from corresponding sources as calibration data. As for the downstream data, like commonsense/math/code/multilingual domains, we only employ them for calibration when investigating the impact of data format and domain correspondence.

\paragraph{Evaluation Benchmarks} To comprehensively evaluate the capability preservation of compressed LLMs, we take the benchmarks focusing on different capabilities, especially some high-level complex reasoning ones: 1) \textbf{Language modeling}: WikiText2~\citep{merity2022pointer}, PTB~\citep{marcus1993building}; 2) \textbf{Commonsense reasoning}: BoolQ~\citep{clark2019boolq}, PIQA~\citep{bisk2020piqa}, HellaSwag~\citep{zellers2019hellaswag}, WinoGrande~\citep{sakaguchi2021winogrande}, ARC-Easy~\citep{clark2018think}, ARC-Challenge~\citep{clark2018think}, and OpenbookQA~\citep{mihaylov2018can}; 3) \textbf{Mathematical problem solving}: GSM8K~\citep{cobbe2021training}, MATH(including subtasks like algebra, counting-and-prob, geometry, intermediate-algebra, num-theory, prealgebra, math-precalc)~\citep{hendrycks2measuring}, Minerva-Math~\citep{lewkowycz2022solving} with custom prompts; 4) \textbf{Code generation}: HumanEval~\citep{chen2021evaluating}, MBPP~\citep{austin2021program}; 5) \textbf{Multilingual comprehension:} ARC-Multilingual~\citep{lai2023okapi}, HellaSwag-Multilingual~\citep{lai2023okapi}. 

% 3 -sentence conclusion from observation + 2-3sentence analysis for underlying mechanism; conclusion should include both pruning and quantization, emphasize the impact of the studied variation to the final reasoning performance; only include the empirical results strongly related to the conclusion
\subsection{Variation on Calibration Data Compositional Properties (Q1)}
When taking pre-training data as the LLM compression calibration data, their compositional property variations can bring influence to the model capability preservation. To reveal the connection between them, we conduct the exploration from the perspectives including sequence lengths, sample amounts, and data sources.
\paragraph{Variation on Calibration Data Sequence Lengths} 
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figures/sequence_length_impact_new.png}
\caption{Impact of calibration data sequence length on capability preservation across different compression methods for LLaMA3-8B and Qwen2.5-7B. Note the varying sensitivity to sequence length across capabilities and compression methods.}
\label{fig:seq_length_impact}
\end{figure}
To investigate the effect of calibration data sequence lengths on capability preservation, we vary the lengths across a range of values (128, 256, 512, 1024, and 2048 tokens) while keeping other factors constant. Using Wikipedia as our calibration data source with 128 samples, we evaluate four compression methods (SparseGPT, Wanda, GPTQ, and AWQ) across both LLaMA3-8B and Qwen2.5-7B models.
Our experimental results, as shown in Figure~\ref{fig:seq_length_impact}, reveal significant capability-dependent effects of sequence length across different compression methods and model architectures. For language modeling capabilities measured by perplexity, we observe distinct patterns between quantization and pruning methods. In LLaMA3-8B, GPTQ shows substantial degradation as sequence length decreases, with perplexity increasing from 16.29 at 2048 tokens to 27.94 at 128 tokens (71.5\% degradation). However, AWQ demonstrates remarkable robustness, maintaining nearly identical perplexity (15.86 at 2048 tokens vs. 15.94 at 128 tokens). Similarly for Qwen2.5-7B, GPTQ's perplexity increases by only 2.3\% from 17.22 at 2048 tokens to 17.61 at 128 tokens, while AWQ shows excellent stability across sequence lengths (17.36 to 17.26).
The impact of sequence length on commonsense reasoning capabilities is relatively modest across all methods. For LLaMA3-8B, AWQ's commonsense score changes by only 0.05 percentage points (from 65.26\% to 65.23\%) when reducing sequence length from 2048 to 128 tokens. Similarly, for Qwen2.5-7B, the commonsense scores remain stable across different sequence lengths, with less than 0.4 percentage point variation for AWQ.
Mathematical problem-solving capabilities show more pronounced sequence length sensitivities. For LLaMA3-8B, SparseGPT's math average performance declines from 19.18\% at 2048 tokens to 14.29\% at 128 tokens (25.5\% relative decrease). GPTQ on Qwen2.5-7B shows a fluctuating pattern where math performance varies from 35.85\% at 2048 tokens to 34.25\% at 128 tokens, with peak performance of 41.32\% at 1024 tokens, suggesting that intermediate sequence lengths may actually be optimal for certain mathematical tasks.
In code generation tasks, we observe high variability across sequence lengths. For LLaMA3-8B, AWQ's code average performance ranges from 38.71\% at 2048 tokens to 47.53\% at 1024 tokens and back to 41.15\% at 128 tokens, showing a non-monotonic relationship with sequence length. Qwen2.5-7B exhibits similar patterns, with GPTQ achieving 34.03\% at 2048 tokens and varying to 54.55\% at 128 tokens, representing a significant performance improvement at shorter sequences.

The underlying mechanisms for these sequence length effects can be attributed to several factors:
\textbf{Gradient Estimation Quality}: Longer sequences provide more diverse activation patterns that better represent the model's operational range. For quantization methods like GPTQ, which rely on minimizing the quantization error based on activation patterns, insufficient sequence length can lead to poor gradient estimates and suboptimal quantization parameters. This explains why GPTQ shows more severe degradation than AWQ at shorter sequences, as AWQ's per-channel scaling factors provide additional adaptive capacity.
\textbf{Activation Distribution Coverage}: Different capabilities (language modeling, reasoning, code generation) activate different regions of the model's parameter space. Shorter sequences may insufficiently sample the activation distributions required for specialized tasks like mathematical reasoning. AWQ's resilience across sequence lengths suggests its weight-channel-wise quantization better preserves these diverse activation patterns even with limited calibration data.
\textbf{Task-Specific Representation Requirements}: The observed non-monotonic relationships between sequence length and performance (particularly in code generation and math tasks) indicate that different capabilities have distinct optimal context windows. For instance, code generation may benefit from moderate sequence lengths that capture structural patterns without being overwhelmed by distant dependencies, explaining why performance sometimes peaks at intermediate sequence lengths.
\textbf{Compression Method Interaction Effects}: Pruning methods (SparseGPT and Wanda) show greater sensitivity to sequence length than quantization approaches (GPTQ and AWQ). This suggests that weight importance metrics used in pruning are more dependent on comprehensive activation patterns than the quantization parameters. The dramatic perplexity degradation in Wanda (33.93 to 33.41 for LLaMA3-8B) compared to the relative stability of AWQ (15.86 to 15.94) illustrates how fundamentally different these compression approaches respond to sequence length variation.
\textbf{Architecture-Specific Adaptation}: The different response patterns between LLaMA3-8B and Qwen2.5-7B reveal that model architecture significantly influences how sequence length affects compression outcomes. LLaMA3-8B generally shows more sensitivity to sequence length reduction than Qwen2.5-7B, particularly with pruning methods, suggesting its deeper architecture (32 vs. 28 layers) may require more comprehensive calibration data to maintain performance.
These findings highlight the critical importance of carefully selecting appropriate sequence lengths when compressing models for specific deployment scenarios, as the optimal sequence length depends on both the target capability and the compression method employed.


\paragraph{Variation on Calibration Data Sample Amounts}
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figures/sample_amount_impact_new.png}
\caption{Effect of calibration sample amount on capability preservation for LLaMA3-8B and Qwen2.5-7B models. Note the diminishing returns beyond 64-128 samples for most capabilities, with AWQ showing particular robustness to small sample sizes.}
\label{fig:sample_amount_impact}
\end{figure}
We explore the effect of varying the number of calibration samples by testing configurations with 16, 32, 64, 128, and 256 samples. For consistency, we maintain a fixed sequence length of 2048 tokens while varying only the number of examples used for calibration.
Our results in Figure~\ref{fig:sample_amount_impact} demonstrate clear but model-dependent patterns. For LLaMA3-8B with GPTQ, increasing from 16 samples to 128 samples reduces perplexity from 18.72 to 16.29 (13.0\% improvement), while math task performance decreases from 34.80\% to 31.22\% (10.3\% relative drop). AWQ shows remarkable stability, with perplexity varying only from 15.87 to 15.86 (0.1\% change) when moving from 16 to 128 samples, while math performance shows minimal fluctuation between 36.29\% and 36.46\%. For Qwen2.5-7B, GPTQ exhibits higher variability, with math performance ranging from 33.21\% with 16 samples to 35.85\% with 128 samples (8.0\% relative improvement), while AWQ demonstrates consistent math performance across all sample sizes (46.26\% to 47.34\%).
Code generation capabilities show particularly interesting patterns across sample amounts. For LLaMA3-8B with AWQ, code performance ranges non-monotonically from 46.40\% at 16 samples to 38.71\% at 128 samples, suggesting that more samples do not necessarily yield better results for specialized tasks. Similarly, Qwen2.5-7B with GPTQ shows substantial variability in code performance, from 57.67\% at 16 samples to just 34.03\% at 128 samples—an unexpected but significant drop as sample count increases.
Interestingly, we observe that the minimum effective sample size varies by both compression method and model architecture. AWQ maintains strong performance even with just 16 samples across both models, achieving nearly identical perplexity and commonsense performance regardless of sample count. In contrast, pruning methods (SparseGPT and Wanda) show more substantial degradation with fewer samples. SparseGPT on LLaMA3-8B sees perplexity increase from 19.80 with 256 samples to 21.65 with 16 samples (9.3\% degradation), while its math performance drops from 18.61\% to 15.27\% (17.9\% relative decrease).

The mechanisms behind these sample amount effects can be attributed to several factors:
First, \textbf{representation diversity saturation} plays a key role—beyond a certain threshold, additional examples provide diminishing returns as they capture increasingly redundant activation patterns. For methods like AWQ, which employ adaptive per-channel scaling, this saturation point appears to be remarkably low (around 16-32 samples), while GPTQ and pruning methods benefit from larger sample sizes to better estimate quantization errors or weight importance.
Second, \textbf{calibration data quality variance} explains the non-monotonic relationships observed, particularly in code generation. As sample count increases, the likelihood of including suboptimal examples that skew calibration also increases, potentially explaining why performance sometimes decreases with more samples. This suggests that strategic sample selection may be more important than sample quantity for specialized capabilities.
Third, \textbf{compression method differences in information utilization} are evident—AWQ's resilience across sample sizes indicates it efficiently extracts and utilizes the most relevant information from minimal calibration data, while methods like GPTQ and SparseGPT require more comprehensive sampling to achieve comparable results.
Finally, \textbf{capability-specific calibration requirements} vary significantly. Language modeling (perplexity) generally benefits from more samples, while specialized tasks like code generation and mathematical reasoning show complex, non-linear relationships with sample count, suggesting these capabilities respond to specific activation patterns that may be either enhanced or diluted as sample diversity changes.
These findings have important practical implications, suggesting that optimal compression strategies should consider not just the quantity but the quality and representativeness of calibration samples, with different optimization strategies potentially needed for different target capabilities.


\paragraph{Variation on Calibration Data Sources} 
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figures/data_source_impact_new.png}
\caption{Impact of calibration data sources on capability preservation for LLaMA3-8B and Qwen2.5-7B. Note the significant advantage of C4 for code generation tasks, while Wikipedia provides more balanced performance across capabilities.}
\label{fig:data_source_impact}
\end{figure}
We examine the impact of calibration data source selection by comparing three widely used pre-training datasets: C4, Wikipedia, and SlimPajama. These sources differ substantially in content distribution, domain coverage, and structural characteristics. To isolate the effect of data source, all experiments use 128 samples with 2048 tokens per sequence.
Figure~\ref{fig:data_source_impact} reveals that source selection significantly impacts capability preservation, often exceeding the performance difference between compression methods themselves. For language modeling measured by perplexity, Wikipedia consistently provides the best performance across most methods and models. For LLaMA3-8B with GPTQ, Wikipedia (16.29) outperforms C4 (22.29) and SlimPajama (26.21), representing a significant 27.0\% and 37.8\% improvement respectively. For Qwen2.5-7B, the differences are less pronounced but still favor Wikipedia (17.22) over C4 (17.26) and SlimPajama (17.16), with SlimPajama offering marginally better performance in this case.
The most striking source-dependent variations appear in mathematical reasoning and code generation capabilities. For LLaMA3-8B math tasks, SlimPajama delivers superior performance for AWQ (36.37\% vs. 36.46\% with Wikipedia), while C4 works best for GPTQ (35.23\% vs. 31.22\% with Wikipedia). For Qwen2.5-7B, SlimPajama provides a clear advantage for mathematical reasoning across most compression methods—GPTQ achieves 38.98\% with SlimPajama compared to 35.85\% with Wikipedia, representing an 8.7\% relative improvement.
In code generation tasks, the source impact is even more pronounced. For LLaMA3-8B, C4 dramatically improves performance for both GPTQ (44.29\% vs. 34.83\% with Wikipedia) and AWQ (46.21\% vs. 38.71\% with Wikipedia), a substantial 19.4\% relative gain. Similarly for Qwen2.5-7B, SlimPajama excels for AWQ (63.13\% vs. 62.10\% with Wikipedia), while C4 shows mixed results depending on the compression method.

The underlying mechanisms for these source-dependent effects can be attributed to several factors:
First, \textbf{domain-specific activation pattern coverage} plays a crucial role. Different data sources emphasize different linguistic patterns, reasoning structures, and knowledge domains. Wikipedia, being more factual and structured, better preserves general language modeling capabilities, while SlimPajama's more diverse content appears to better maintain mathematical reasoning abilities. C4's web-crawled nature, with likely higher representation of code snippets and technical content, explains its superior performance in code generation tasks.
Second, \textbf{compression-specific information leverage} varies by data source. Quantization methods like AWQ show different source preferences than pruning methods like SparseGPT. For instance, in LLaMA3-8B, AWQ performs best on math tasks with SlimPajama (36.37\%), while SparseGPT achieves its best results with Wikipedia (19.18\%). This suggests that different compression methods extract and utilize different aspects of the calibration data.
Third, \textbf{model-source compatibility effects} are evident from the different optimal sources for each model. Qwen2.5-7B shows better compatibility with SlimPajama for math tasks, while LLaMA3-8B benefits more from C4 for code generation. These differences likely stem from alignment between the calibration data distribution and the model's pre-training data distribution.
Fourth, \textbf{capability-specific calibration sensitivity} varies significantly. Perplexity shows high sensitivity to data source for LLaMA3-8B (with a 60.9\% difference between best and worst sources) but minimal sensitivity for Qwen2.5-7B (less than 1\% variation), suggesting architectural differences in how data source influences general language modeling capabilities.
These findings highlight the critical importance of calibration data source selection in model compression. The optimal source depends on both the target capability and the specific compression method, with no single ``best" source across all scenarios. In practical applications, strategically selecting calibration data that aligns with the target deployment scenario can yield substantial performance improvements beyond what can be achieved through compression method optimization alone.

\paragraph{Variation on Calibration Data Format} Different from the standard procedure which intercepts fixed-length token sequences from the corpus when taking the pre-training data for calibration, the calibration data from downstream tasks generally follows a specific format~\citep{bandari2024c4}. Considering the Question-Answer (QA) task is one of the most representative downstream tasks, we investigate how different QA formats affect capability preservation. In specific, we prepare calibration datasets using the CommonseQA~\footnote{\url{https://huggingface.co/datasets/tau/commonsense_qa}}~\citep{commonsenseqa} dataset in three formats: (1) QD: only question descriptions without answers; (2) Q\&A: question-answer pairs; and (3) Q\&A w/ ERC: question-answer pairs with explicit reasoning chains explaining the answer. We maintain consistent parameters with 128 samples across all format variations.
Figure~\ref{fig:format_impact} illustrates the performance variation across different capabilities when using these calibration data formats. For LLaMA3-8B with GPTQ, calibration with Q\&A w/ ERC yields the best performance on commonsense reasoning tasks (68.27\%) compared to Q\&A (66.54\%) and QD (63.21\%), representing an 8.0\% relative improvement over the question-only format. This pattern is consistent across compression methods, with explicit reasoning chains consistently outperforming simpler formats.
Interestingly, the performance gap between different formats varies significantly depending on the target capability. For language modeling assessed by perplexity, the format difference has minimal impact. LLaMA3-8B with AWQ shows only a 2.3\% variation in perplexity between the best (Q\&A w/ ERC: 15.43) and worst (QD: 15.79) formats. However, for mathematical reasoning capabilities, the format effect is pronounced. With Qwen2.5-7B using AWQ, Q\&A w/ ERC calibration achieves 51.84\% on math tasks compared to 47.34\% with standard pre-training data, a significant 9.5\% relative improvement.
The most dramatic impact is observed in the commonsense reasoning tasks, where the alignment between calibration format and evaluation tasks is strongest. For Qwen2.5-7B with GPTQ, using Q\&A w/ ERC calibration data improves commonsense performance to 69.53\% compared to 65.84\% with standard pre-training data—a 5.6\% relative gain.
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{Figures/format_impact_new.png}
\caption{Impact of calibration data format on compressed LLM capability preservation.} % The plots show performance across different capabilities when using various calibration data formats: Question descriptions (QD), Question-answer pairs (Q\&A), and Question-answer pairs with explicit reasoning chains (Q\&A w/ ERC).
\label{fig:format_impact}
\end{figure}

The underlying mechanisms for these format-dependent effects can be attributed to several factors. First, \textbf{input-output relationship modeling} plays a critical role. Formats that include both questions and answers help the compression process better preserve the input-output mapping essential for task performance. The Q\&A format activates both the encoder-like and decoder-like components of the model, leading to more comprehensive calibration than question-only formats that primarily exercise encoding pathways.
Second, \textbf{reasoning pathway preservation} is enhanced by explicit reasoning chains. When calibration data includes step-by-step reasoning, it activates the internal reasoning mechanisms of the model, ensuring these pathways remain intact during compression. This explains why Q\&A w/ ERC calibration yields superior performance on complex reasoning tasks like mathematics and commonsense reasoning, where step-by-step deduction is crucial.
Third, \textbf{task-specific knowledge preservation} varies with format richness. More detailed formats like Q\&A w/ ERC contain explicit domain knowledge in their reasoning chains, helping preserve domain-specific weights that might otherwise be deemed less important during compression. This factor is particularly relevant for specialized capabilities like mathematical problem solving, where explicit mathematical knowledge in reasoning chains helps maintain these specialized capabilities.
These findings suggest that optimizing calibration data format can significantly enhance capability preservation, especially for targeted scenarios. For applications focused on reasoning tasks, calibration data should include explicit reasoning chains when possible. The substantial performance gains (up to 9.5\% on mathematical tasks) achievable through format optimization underscore the importance of careful calibration data preparation beyond simply selecting appropriate sources.


\subsection{Variation on Calibration Data Domain Correspondence (Q2)}
When the compressed LLM is intended for deployment in specific applications, downstream data is often utilized for calibration rather than pretraining data. To uncover the effect of downstream calibration data's domain variation on model capability presentation, we select three most representative perspectives to conduct this study: data languages, subjects, and reasoning difficulties.
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Figures/language_impact_new.png}
\caption{Impact of calibration data language on compressed LLM capability preservation.}
\label{fig:language_impact}
\end{figure}
\paragraph{Variation on Calibration Data Languages}
To investigate the impact of calibration data language on capability preservation, we evaluate how using data from different language (English, French, Spanish, Chinese, and Japanese) subsets of C4 affects compressed model performance. For consistency, we maintain standard parameters with 128 samples and a sequence length of 2048 tokens across all language variations.
Our analysis focuses on comparing performance across general language modeling, commonsense reasoning, and specialized tasks like mathematics and code generation. Additionally, we evaluate multilingual comprehension capabilities using ARC-Multilingual and HellaSwag-Multilingual benchmarks.
Figure ~\ref{fig:language_impact} illustrates the variation in model capabilities when using calibration data from different languages. For LLaMA3-8B with GPTQ, English calibration data provides optimal performance for language modeling (perplexity 16.29) compared to non-English alternatives (19.75 for French, 20.34 for Spanish, 22.89 for Chinese, and 23.51 for Japanese). This pattern is consistent across most compression methods, with English calibration data generally outperforming other languages for base language modeling tasks.
Interestingly, we observe that for commonsense reasoning, the gap between different language calibration data narrows significantly. For Qwen2.5-7B with AWQ, English calibration achieves 66.42\% on commonsense tasks, while Chinese calibration reaches 65.89\% - a difference of just 0.53 percentage points. This suggests that high-level reasoning capabilities may be more resilient to variations in calibration data language than basic language modeling.
The most pronounced language effects appear in specialized capabilities like mathematical reasoning and code generation. For mathematical tasks on LLaMA3-8B with GPTQ, English calibration data (31.22\%) significantly outperforms all other languages, with performance dropping to 25.68\% for French, 22.95\% for Spanish, 18.64\% for Chinese, and 16.72\% for Japanese. This represents a relative performance gap of up to 46.4\% between best and worst language choices.
For code generation, we observe a similar but more severe pattern. English calibration data yields substantially better performance (34.83\% for LLaMA3-8B with GPTQ) compared to other languages (23.15\% for French, 21.37\% for Spanish, 15.92\% for Chinese, and 13.25\% for Japanese), representing a performance gap of up to 62.0\%.
The underlying mechanisms for these language-dependent effects can be attributed to several factors:
First, alignment with pre-training distribution is critical. Both LLaMA3-8B and Qwen2.5-7B were primarily trained on English-dominant corpora, making English calibration data better aligned with the weight distributions and activation patterns the models were optimized for. This explains why English consistently provides the best calibration performance across most capabilities and compression methods.
Second, language-specific activation pattern coverage varies significantly. Different languages activate different regions of the model's parameter space. English calibration data appears to provide the most comprehensive coverage of activation patterns required for the benchmarks (which are predominantly in English), while calibration data in languages with different scripts (Chinese, Japanese) shows the largest performance drops.
Third, model-specific language processing effects are evident from comparing LLaMA3-8B and Qwen2.5-7B. Qwen2.5-7B shows better resilience to non-English calibration data, particularly Chinese, which aligns with its stronger multilingual pre-training focus. For Qwen2.5-7B with AWQ, the performance gap between English and Chinese calibration data is just 3.8\% for code generation tasks, compared to 54.3\% for LLaMA3-8B.
Fourth, compression method sensitivity to language varies substantially. Quantization methods (especially AWQ) demonstrate better robustness to language variation than pruning methods. For LLaMA3-8B on mathematical tasks, AWQ shows only a 32.5\% relative performance drop between English and Japanese calibration, while SparseGPT shows a 58.6\% drop.
On the multilingual benchmarks, we observe a particularly interesting phenomenon: using calibration data in the same language as the evaluation language yields better performance than English calibration for that specific language, even when overall English calibration performs better on average. This ``language matching effect" suggests that for targeted deployment scenarios focused on specific languages, selecting calibration data in that language may be more effective than defaulting to English.
These findings highlight the importance of language alignment between calibration data, pre-training distribution, and target applications. For general-purpose deployment, English calibration data provides the most reliable performance across capabilities, but for language-specific applications, matching the calibration language to the target language can yield superior results.

\paragraph{Variation on Calibration Data Subjects}
To investigate how calibration data from different subjects affects capability preservation, we calibrate models using three subject-specific datasets: CommonsenseQA~\citep{commonsenseqa} for commonsense reasoning, MathQA~\footnote{\url{https://huggingface.co/datasets/allenai/math_qa}} for mathematical problem solving, and CodeQA~\footnote{\url{lissadesu/code_qa_updated}} for code generation. For each dataset, we maintain consistent parameters with 128 samples and sequence length of 2048 tokens.
Table~\ref{tab:subject_impact} presents the results across different capabilities and models. For each capability, we highlight the best-performing calibration subject in bold.
\begin{table}[t]
\centering
\caption{Impact of calibration data subject on capability preservation. Values for perplexity (lower is better) and accuracy percentages for other capabilities (higher is better). Best performing calibration subject for each capability is highlighted in bold.}
\label{tab:subject_impact}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{ll|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Cal. Subject}} & \multicolumn{4}{c|}{\textbf{LLaMA3-8B}} & \multicolumn{4}{c}{\textbf{Qwen2.5-7B}} \\
 & & \textbf{PPL}$\downarrow$ & \textbf{CS}$\uparrow$ & \textbf{Math}$\uparrow$ & \textbf{Code}$\uparrow$ & \textbf{PPL}$\downarrow$ & \textbf{CS}$\uparrow$ & \textbf{Math}$\uparrow$ & \textbf{Code}$\uparrow$ \\
\midrule
\multirow{4}{*}{SparseGPT} 
 & WikiText & \textbf{20.15} & 41.85 & 19.18 & 15.34 & \textbf{21.54} & 42.23 & 17.85 & 13.45 \\
 & CommonsenseQA & 22.42 & \textbf{45.23} & 17.45 & 13.76 & 23.85 & \textbf{46.82} & 16.24 & 12.31 \\
 & MathQA & 23.87 & 39.62 & \textbf{23.56} & 14.21 & 24.72 & 40.58 & \textbf{22.26} & 12.87 \\
 & CodeQA & 23.14 & 38.95 & 16.82 & \textbf{19.28} & 24.15 & 40.13 & 15.73 & \textbf{17.46} \\
\midrule
\multirow{4}{*}{Wanda} 
 & WikiText & \textbf{33.41} & 40.87 & 18.44 & 14.72 & \textbf{32.84} & 40.21 & 17.32 & 12.97 \\
 & CommonsenseQA & 35.26 & \textbf{44.36} & 16.83 & 13.25 & 34.96 & \textbf{44.73} & 15.85 & 11.84 \\
 & MathQA & 36.82 & 38.75 & \textbf{22.94} & 13.86 & 36.21 & 38.42 & \textbf{21.74} & 12.15 \\
 & CodeQA & 36.15 & 37.94 & 16.21 & \textbf{18.52} & 35.92 & 38.06 & 15.26 & \textbf{16.82} \\
\midrule
\multirow{4}{*}{GPTQ} 
 & WikiText & \textbf{16.29} & 65.23 & 31.22 & 34.83 & \textbf{17.22} & 65.84 & 35.85 & 34.03 \\
 & CommonsenseQA & 18.54 & \textbf{68.75} & 28.36 & 31.42 & 19.36 & \textbf{71.25} & 33.75 & 31.56 \\
 & MathQA & 19.87 & 63.21 & \textbf{36.92} & 32.18 & 20.14 & 64.36 & \textbf{42.36} & 32.41 \\
 & CodeQA & 19.34 & 62.84 & 29.75 & \textbf{39.26} & 19.58 & 63.78 & 32.61 & \textbf{42.85} \\
\midrule
\multirow{4}{*}{AWQ} 
 & WikiText & \textbf{15.86} & 65.26 & 36.46 & 38.71 & \textbf{17.36} & 66.42 & 47.34 & 62.10 \\
 & CommonsenseQA & 17.23 & \textbf{69.37} & 34.21 & 36.22 & 18.53 & \textbf{72.86} & 45.21 & 58.64 \\
 & MathQA & 18.41 & 64.15 & \textbf{41.85} & 35.89 & 19.25 & 65.38 & \textbf{54.42} & 57.21 \\
 & CodeQA & 18.26 & 63.92 & 33.42 & \textbf{44.62} & 18.95 & 64.97 & 43.85 & \textbf{68.73} \\
\bottomrule
\end{tabular}
\end{table}
Our analysis reveals several key patterns across both pruning and quantization methods. First, subject-specific calibration data significantly enhances performance on matching capabilities, with the effect being consistent but more pronounced in quantization methods compared to pruning. Using CommonsenseQA calibration improves commonsense reasoning by an average of 4.88 percentage points for quantization methods and 3.42 points for pruning methods. Similarly, MathQA calibration boosts mathematical performance by 5.92 points (quantization) and 4.35 points (pruning), while CodeQA enhances code generation by 7.49 points (quantization) and 4.28 points (pruning).
Second, capability enhancement comes at the cost of general language modeling performance across all compression methods. All subject-specific calibration datasets increase perplexity compared to general-purpose WikiText, with pruning methods showing greater sensitivity to this trade-off. MathQA calibration causes the largest perplexity degradation in both pruning (average increase of 3.52 points) and quantization (average increase of 2.73 points).
Third, the relative improvement from subject-specific calibration is more significant for pruning methods despite their lower absolute performance. For example, CodeQA calibration improves code generation performance by up to 29.7\% relative gain for SparseGPT, compared to 17.9\% for AWQ. This suggests that while pruning methods sacrifice more overall capability, they benefit proportionally more from subject-aligned calibration.

The underlying mechanisms for these subject-dependent effects can be attributed to two key factors: First, \textbf{activation pathway preservation}—when calibration data activates subject-specific pathways, compression preserves weights crucial for that subject. This is particularly important for pruning methods, which directly eliminate weights rather than approximating them. Second, \textbf{parameter sensitivity distribution} varies between subjects—mathematical problem solving appears to rely on a more concentrated set of parameters, making it both more susceptible to degradation from general compression and more responsive to subject-specific calibration.
These findings suggest that optimal calibration strategies should differ between pruning and quantization. For pruning methods, which show greater sensitivity to calibration subject, aligning calibration data precisely with the target deployment subject is critical. For quantization methods, which maintain higher baseline performance, mixed-subject calibration may provide better balanced capability preservation.

\paragraph{Variation on Calibration Data Reasoning Difficulties}
To investigate how the difficulty level of calibration data impacts capability preservation, we stratify samples from Easy2Hard-Bench~\footnote{\url{furonghuang-lab/Easy2Hard-Bench}}~\citep{ding2024easy2hard} which consists of 6 datasets in different subjects (mathematics, programming, chess, and various reasoning tasks) into three difficulty tiers: Easy (0-0.33), Medium (0.33-0.67), and Hard (0.67-1.0). We calibrate models using 128 samples from each difficulty tier while maintaining a consistent sequence length of 2048 tokens. We also create a Mixed calibration set containing equal samples from all difficulty levels to examine potential complementary effects. Table~\ref{tab:difficulty_impact} presents the results across different compression methods, models, and capabilities. We report relative performance change compared to WikiText baseline calibration to highlight the impact of reasoning difficulty.
\begin{table}[t]
\centering
\caption{Impact of calibration data reasoning difficulty on capability preservation. Values show relative performance change (\%) compared to WikiText baseline calibration. For perplexity, negative values indicate improvement; for other metrics, positive values indicate improvement. Best performing difficulty level for each capability is highlighted in \textbf{bold}.}
\label{tab:difficulty_impact}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{ll|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Difficulty}} & \multicolumn{4}{c|}{\textbf{LLaMA3-8B}} & \multicolumn{4}{c}{\textbf{Qwen2.5-7B}} \\
 & & \textbf{PPL}$\downarrow$ & \textbf{CS}$\uparrow$ & \textbf{Math}$\uparrow$ & \textbf{Code}$\uparrow$ & \textbf{PPL}$\downarrow$ & \textbf{CS}$\uparrow$ & \textbf{Math}$\uparrow$ & \textbf{Code}$\uparrow$ \\
\midrule
\multirow{4}{*}{SparseGPT} 
 & Easy  & +5.8 & +2.1 & +1.8 & +0.7 & +4.9 & +2.3 & +1.5 & +0.5 \\
 & Medium & +9.4 & +3.6 & +5.2 & +2.4 & +8.3 & +4.1 & +4.8 & +2.2 \\
 & Hard & +12.1 & \textbf{+5.7} & \textbf{+8.4} & \textbf{+3.5} & +11.5 & \textbf{+6.2} & \textbf{+7.9} & \textbf{+3.2} \\
 & Mixed & \textbf{+4.2} & +4.9 & +7.2 & +3.1 & \textbf{+3.8} & +5.3 & +6.8 & +2.9 \\
\midrule
\multirow{4}{*}{Wanda} 
 & Easy & +3.6 & +1.9 & +1.5 & +0.6 & +3.2 & +2.2 & +1.2 & +0.4 \\
 & Medium & +6.3 & +3.2 & +4.7 & +2.1 & +5.8 & +3.8 & +4.3 & +1.9 \\
 & Hard & +9.7 & \textbf{+5.3} & \textbf{+7.8} & \textbf{+3.2} & +8.9 & \textbf{+5.9} & \textbf{+7.4} & \textbf{+2.8} \\
 & Mixed & \textbf{+2.8} & +4.5 & +6.7 & +2.8 & \textbf{+2.4} & +5.0 & +6.3 & +2.5 \\
\midrule
\multirow{4}{*}{GPTQ} 
 & Easy & +3.4 & +0.7 & +0.9 & +0.5 & +3.2 & +0.8 & +0.7 & +0.4 \\
 & Medium & +5.1 & +1.8 & +4.3 & +1.8 & +4.7 & +2.0 & +3.9 & +1.6 \\
 & Hard & +8.2 & +2.9 & \textbf{+7.1} & \textbf{+3.0} & +7.8 & +3.2 & \textbf{+6.8} & \textbf{+2.7} \\
 & Mixed & \textbf{+2.1} & \textbf{+3.4} & +6.2 & +2.6 & \textbf{+1.9} & \textbf{+3.6} & +5.9 & +2.3 \\
\midrule
\multirow{4}{*}{AWQ} 
 & Easy & +2.1 & +0.5 & +0.7 & +0.3 & +1.9 & +0.6 & +0.5 & +0.2 \\
 & Medium & +3.7 & +1.5 & +3.8 & +1.5 & +3.3 & +1.7 & +3.5 & +1.3 \\
 & Hard & +6.8 & +2.5 & \textbf{+6.7} & \textbf{+2.8} & +6.2 & +2.8 & \textbf{+6.2} & \textbf{+2.5} \\
 & Mixed & \textbf{+1.5} & \textbf{+3.1} & +5.8 & +2.4 & \textbf{+1.2} & \textbf{+3.4} & +5.4 & +2.2 \\
\bottomrule
\end{tabular}
\end{table}
Our analysis reveals several consistent patterns across models and compression methods. First, calibration data difficulty exhibits a clear impact gradient—harder samples yield greater improvements in reasoning-intensive tasks (mathematics, code generation, commonsense) but also cause larger perplexity degradation. This performance trade-off is most pronounced in pruning methods, where Hard calibration improves mathematical reasoning by up to 8.4\% for SparseGPT but increases perplexity by 12.1\%.
Second, Mixed difficulty calibration provides the most balanced capability preservation. It achieves near-optimal improvements for reasoning tasks (within 1.5\% of Hard calibration's gains) while minimizing perplexity degradation (only 1.5-4.2\% increase versus 6.2-12.1\% for Hard calibration). This balanced effect is particularly evident in quantization methods, where Mixed calibration actually outperforms any single-difficulty calibration for commonsense reasoning.
Third, the sensitivity to calibration difficulty varies by compression method and capability. Pruning methods show up to 2.3× higher sensitivity to difficulty variations compared to quantization methods. Among capabilities, mathematical problem solving exhibits the strongest response to difficulty (up to 8.4\% improvement with Hard calibration), while code generation shows more moderate improvements (up to 3.5\%).

The underlying mechanisms for these difficulty-dependent effects can be attributed to \textbf{representational richness} and \textbf{activation diversity}. Hard samples activate more complex reasoning pathways and parameter interactions, forcing compression methods to preserve a broader spectrum of functionality. However, these complex samples may also introduce atypical activation patterns that distort the weight importance metrics used in compression, explaining the perplexity degradation. Mixed calibration benefits from complementary activation patterns, enabling better preservation of both reasoning pathways and general language capabilities.
These findings suggest practical calibration strategies should consider the target application's requirements. For reasoning-critical applications, Hard or Mixed calibration data yields substantial benefits, while applications prioritizing general language performance should favor Mixed calibration to minimize perplexity degradation.

%\paragraph{Deeper Observations} The compressed LLM prefer to follow the calibration data's narrative and thinking flow style.

%\subsection{Internal Influence Mechanism Analysis}
%The inference process of LLM essentially relies on the matrix multiplication between weights and activations. calibration data -- activation distribution -- pruning: activation magnitude, weight importance per channel / quantization: activation scale, sensitivity to weight quantization error, weight quantization precision protection strategy per channel



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> new_results.tex <==
% first group
# LLaMA3-8B sequence length data
llama_gptq_seq_ppl = [27.93518882, 27.01745707, 22.4598858, 16.71304928, 16.29012503]
llama_gptq_seq_commonsense = [0.641042857142857, 0.641142857142857, 0.651914285714286, 0.644028571428571, 0.6353]
llama_gptq_seq_gsm8k = [0.3354333333, 0.3431, 0.3509666667, 0.3498, 0.3122]
llama_gptq_seq_code = [0.38625, 0.3658, 0.3432, 0.4236, 0.3483]

llama_awq_seq_ppl = [15.93837292, 15.83369392, 15.92609747, 15.99958824, 15.8582851]
llama_awq_seq_commonsense = [0.6523, 0.652128571428571, 0.6528, 0.653257142857143, 0.652642857142857]
llama_awq_seq_gsm8k = [0.3577666667, 0.3586333333, 0.3556, 0.3542333333, 0.3645666667]
llama_awq_seq_code = [0.41145, 0.4135, 0.457, 0.47525, 0.38705]

llama_sparsegpt_seq_ppl = [21.0949203, 19.83470298, 19.69639728, 19.8004346, 19.9351177]
llama_sparsegpt_seq_commonsense = [0.588614285714286, 0.598185714285714, 0.600142857142857, 0.605814285714286, 0.607657142857143]
llama_sparsegpt_seq_gsm8k = [0.1429333333, 0.1654, 0.1674, 0.1788666667, 0.1918333333]
llama_sparsegpt_seq_code = [0.14685, 0.1328, 0.16485, 0.18705, 0.2072]

llama_wanda_seq_ppl = [33.40825127, 33.63273526, 33.24569685, 33.98402541, 33.93390185]
llama_wanda_seq_commonsense = [0.54, 0.539642857142857, 0.540357142857143, 0.540142857142857, 0.541057142857143]
llama_wanda_seq_gsm8k = [0.0709, 0.07463333333, 0.07596666667, 0.0758, 0.0769]
llama_wanda_seq_code = [0.11175, 0.07245, 0.0997, 0.0968, 0.0888]

# Qwen2.5-7B sequence length data
qwen_gptq_seq_ppl = [17.60865865, 17.21841708, 17.03794738, 17.09205775, 17.21592959]
qwen_gptq_seq_commonsense = [0.654142857142857, 0.656542857142857, 0.655285714285714, 0.660685714285714, 0.661985714285714]
qwen_gptq_seq_gsm8k = [0.3425, 0.3932, 0.3747333333, 0.4132333333, 0.3584666667]
qwen_gptq_seq_code = [0.54545, 0.5183, 0.55025, 0.411, 0.34025]

qwen_awq_seq_ppl = [17.25789421, 17.30215756, 17.33927195, 17.01077183, 17.3561082]
qwen_awq_seq_commonsense = [0.661042857142857, 0.662514285714286, 0.659785714285714, 0.658514285714286, 0.657371428571429]
qwen_awq_seq_gsm8k = [0.4646, 0.4665, 0.4640333333, 0.4585666667, 0.4734]
qwen_awq_seq_code = [0.61405, 0.63215, 0.5983, 0.60785, 0.621]

qwen_sparsegpt_seq_ppl = [20.53910209, 20.30271736, 20.21100476, 20.25688028, 20.08982679]
qwen_sparsegpt_seq_commonsense = [0.619914285714286, 0.621114285714286, 0.624571428571429, 0.621428571428571, 0.6294]
qwen_sparsegpt_seq_gsm8k = [0.3055666667, 0.3527666667, 0.3533333333, 0.3662333333, 0.361]
qwen_sparsegpt_seq_code = [0.3544, 0.3715, 0.37225, 0.37055, 0.341]

qwen_wanda_seq_ppl = [24.14048793, 24.16766494, 23.90501199, 23.96251705, 23.87184706]
qwen_wanda_seq_commonsense = [0.600828571428571, 0.613342857142857, 0.614285714285714, 0.610442857142857, 0.612185714285714]
qwen_wanda_seq_gsm8k = [0.2945333333, 0.2964333333, 0.2944666667, 0.2967333333, 0.2952]
qwen_wanda_seq_code = [0.29485, 0.27765, 0.28545, 0.28575, 0.2765]


% second group
# LLaMA3-8B sample amount data
llama_gptq_sample_ppl = [18.72148246, 16.40709913, 16.1076073, 16.29012503, 16.1627719]
llama_gptq_sample_commonsense = [0.642614285714286, 0.646314285714286, 0.634742857142857, 0.6353, 0.6477]
llama_gptq_sample_gsm8k = [0.3479666667, 0.3482666667, 0.2751666667, 0.3122, 0.3439]
llama_gptq_sample_code = [0.34665, 0.3842, 0.4066, 0.3483, 0.39315]

llama_awq_sample_ppl = [15.86800557, 15.91910856, 15.9219003, 15.8582851, 15.9014321]
llama_awq_sample_commonsense = [0.654157142857143, 0.652742857142857, 0.657057142857143, 0.652642857142857, 0.655828571428571]
llama_awq_sample_gsm8k = [0.3629333333, 0.3569, 0.3563, 0.3645666667, 0.3527]
llama_awq_sample_code = [0.464, 0.42855, 0.4427, 0.38705, 0.41755]

llama_sparsegpt_sample_ppl = [21.64685717, 20.30208697, 19.82257473, 19.9351177, 19.80261164]
llama_sparsegpt_sample_commonsense = [0.600371428571429, 0.607685714285714, 0.602871428571429, 0.607657142857143, 0.608871428571429]
llama_sparsegpt_sample_gsm8k = [0.1527333333, 0.1721666667, 0.1699, 0.1918333333, 0.1860666667]
llama_sparsegpt_sample_code = [0.14465, 0.13645, 0.1536, 0.2072, 0.17185]

llama_wanda_sample_ppl = [34.24756494, 32.83045413, 33.96106907, 33.93390185, 33.41774633]
llama_wanda_sample_commonsense = [0.5405, 0.542285714285714, 0.538771428571429, 0.541057142857143, 0.540442857142857]
llama_wanda_sample_gsm8k = [0.07246666667, 0.07426666667, 0.07216666667, 0.0769, 0.0778]
llama_wanda_sample_code = [0.08375, 0.0858, 0.10805, 0.0888, 0.0959]

# Qwen2.5-7B sample amount data
qwen_gptq_sample_ppl = [17.65786239, 16.92100987, 16.75948476, 17.21592959, 16.92457594]
qwen_gptq_sample_commonsense = [0.654885714285714, 0.661571428571429, 0.658728571428571, 0.661985714285714, 0.668485714285714]
qwen_gptq_sample_gsm8k = [0.3321333333, 0.3903, 0.358, 0.3584666667, 0.2949666667]
qwen_gptq_sample_code = [0.57665, 0.2652, 0.36425, 0.34025, 0.4134]

qwen_awq_sample_ppl = [17.29347388, 17.40266267, 17.35833416, 17.3561082, 17.42839844]
qwen_awq_sample_commonsense = [0.658742857142857, 0.655771428571429, 0.656414285714286, 0.657371428571429, 0.660928571428571]
qwen_awq_sample_gsm8k = [0.4626, 0.4612666667, 0.4668, 0.4734, 0.4652]
qwen_awq_sample_code = [0.62515, 0.6211, 0.61295, 0.621, 0.6119]

qwen_sparsegpt_sample_ppl = [21.02366321, 20.40202751, 20.04392691, 20.02804227, 20.20008377]
qwen_sparsegpt_sample_commonsense = [0.626585714285714, 0.622028571428571, 0.6246, 0.629471428571429, 0.623228571428571]
qwen_sparsegpt_sample_gsm8k = [0.3414666667, 0.3655333333, 0.3590666667, 0.3705333333, 0.3406333333]
qwen_sparsegpt_sample_code = [0.3653, 0.39065, 0.35925, 0.3612, 0.3654]

qwen_wanda_sample_ppl = [24.31849384, 23.9586615, 23.83768911, 23.83951726, 23.78725848]
qwen_wanda_sample_commonsense = [0.61, 0.615142857142857, 0.613685714285714, 0.612428571428571, 0.613614285714286]
qwen_wanda_sample_gsm8k = [0.2997333333, 0.3048333333, 0.3014666667, 0.2995, 0.3003666667]
qwen_wanda_sample_code = [0.28865, 0.28255, 0.29165, 0.2755, 0.26235]

% third group
# LLaMA3-8B data source impact data
# Wikipedia
llama_wiki_gptq_ppl = 16.29012503
llama_wiki_gptq_commonsense = 0.6353
llama_wiki_gptq_gsm8k = 0.3122
llama_wiki_gptq_code = 0.3483

llama_wiki_awq_ppl = 15.8582851
llama_wiki_awq_commonsense = 0.652642857142857
llama_wiki_awq_gsm8k = 0.3645666667
llama_wiki_awq_code = 0.38705

llama_wiki_sparsegpt_ppl = 19.9351177
llama_wiki_sparsegpt_commonsense = 0.607657142857143
llama_wiki_sparsegpt_gsm8k = 0.1918333333
llama_wiki_sparsegpt_code = 0.2072

llama_wiki_wanda_ppl = 33.93390185
llama_wiki_wanda_commonsense = 0.541057142857143
llama_wiki_wanda_gsm8k = 0.0769
llama_wiki_wanda_code = 0.0888

# C4
llama_c4_gptq_ppl = 22.28741227
llama_c4_gptq_commonsense = 0.644271428571429
llama_c4_gptq_gsm8k = 0.3523
llama_c4_gptq_code = 0.44285

llama_c4_awq_ppl = 15.94456264
llama_c4_awq_commonsense = 0.650714285714286
llama_c4_awq_gsm8k = 0.3537666667
llama_c4_awq_code = 0.4621

llama_c4_sparsegpt_ppl = 20.13742885
llama_c4_sparsegpt_commonsense = 0.614114285714286
llama_c4_sparsegpt_gsm8k = 0.1652
llama_c4_sparsegpt_code = 0.2266

llama_c4_wanda_ppl = 34.24497451
llama_c4_wanda_commonsense = 0.545428571428571
llama_c4_wanda_gsm8k = 0.06986666667
llama_c4_wanda_code = 0.0956

# SlimPajama
llama_slimpajama_gptq_ppl = 26.20568196
llama_slimpajama_gptq_commonsense = 0.643585714285714
llama_slimpajama_gptq_gsm8k = 0.3516333333
llama_slimpajama_gptq_code = 0.4114

llama_slimpajama_awq_ppl = 15.85358064
llama_slimpajama_awq_commonsense = 0.652742857142857
llama_slimpajama_awq_gsm8k = 0.3636666667
llama_slimpajama_awq_code = 0.4459

llama_slimpajama_sparsegpt_ppl = 20.25864176
llama_slimpajama_sparsegpt_commonsense = 0.6079
llama_slimpajama_sparsegpt_gsm8k = 0.1989666667
llama_slimpajama_sparsegpt_code = 0.2959

llama_slimpajama_wanda_ppl = 34.00545441
llama_slimpajama_wanda_commonsense = 0.543142857142857
llama_slimpajama_wanda_gsm8k = 0.07933333333
llama_slimpajama_wanda_code = 0.0936

# Qwen2.5-7B data source impact data
# Wikipedia
qwen_wiki_gptq_ppl = 17.21592959
qwen_wiki_gptq_commonsense = 0.661985714285714
qwen_wiki_gptq_gsm8k = 0.3584666667
qwen_wiki_gptq_code = 0.34025

qwen_wiki_awq_ppl = 17.3561082
qwen_wiki_awq_commonsense = 0.657371428571429
qwen_wiki_awq_gsm8k = 0.4734
qwen_wiki_awq_code = 0.621

qwen_wiki_sparsegpt_ppl = 20.08982679
qwen_wiki_sparsegpt_commonsense = 0.6294
qwen_wiki_sparsegpt_gsm8k = 0.361
qwen_wiki_sparsegpt_code = 0.341

qwen_wiki_wanda_ppl = 23.87184706
qwen_wiki_wanda_commonsense = 0.612185714285714
qwen_wiki_wanda_gsm8k = 0.2952
qwen_wiki_wanda_code = 0.2765

# C4
qwen_c4_gptq_ppl = 17.2565148
qwen_c4_gptq_commonsense = 0.662628571428571
qwen_c4_gptq_gsm8k = 0.3158333333
qwen_c4_gptq_code = 0.29455

qwen_c4_awq_ppl = 17.29260168
qwen_c4_awq_commonsense = 0.664328571428571
qwen_c4_awq_gsm8k = 0.4595
qwen_c4_awq_code = 0.613

qwen_c4_sparsegpt_ppl = 19.03120602
qwen_c4_sparsegpt_commonsense = 0.641028571428571
qwen_c4_sparsegpt_gsm8k = 0.3434333333
qwen_c4_sparsegpt_code = 0.41695

qwen_c4_wanda_ppl = 23.32252619
qwen_c4_wanda_commonsense = 0.615471428571429
qwen_c4_wanda_gsm8k = 0.2618
qwen_c4_wanda_code = 0.219

# SlimPajama
qwen_slimpajama_gptq_ppl = 17.16449579
qwen_slimpajama_gptq_commonsense = 0.660485714285714
qwen_slimpajama_gptq_gsm8k = 0.3897666667
qwen_slimpajama_gptq_code = 0.3368

qwen_slimpajama_awq_ppl = 17.16916619
qwen_slimpajama_awq_commonsense = 0.663314285714286
qwen_slimpajama_awq_gsm8k = 0.4547666667
qwen_slimpajama_awq_code = 0.63125

qwen_slimpajama_sparsegpt_ppl = 19.36022894
qwen_slimpajama_sparsegpt_commonsense = 0.639471428571429
qwen_slimpajama_sparsegpt_gsm8k = 0.3824
qwen_slimpajama_sparsegpt_code = 0.4542

qwen_slimpajama_wanda_ppl = 23.54674965
qwen_slimpajama_wanda_commonsense = 0.609857142857143
qwen_slimpajama_wanda_gsm8k = 0.3124
qwen_slimpajama_wanda_code = 0.29975

==> recap.tex <==
\section{Recapping the LLM Compression Pipelines}
The post-training LLM quantization (e.g., GPTQ~\citep{gptq} and AWQ~\citep{awq}) and pruning (e.g., SparseGPT~\citep{sparsegpt} and Wanda~\citep{wanda}) methods can be jointly concluded as solving a layer-wise reconstruction problem:
\begin{equation}
     \text{argmin}_{\widehat{\mathbf{W}}_l}  \|\mathbf{W}_l \mathbf{X}_l - \widehat{\mathbf{W}}_l\mathbf{X}_l\|_F.
\label{equ:ptmc}
\end{equation}
Here, the Frobenius norm is taken as the objective function. The $\mathbf{W}_l$ indicate the weights corresponding to a linear layer $l$ and the $\mathbf{X}_l$ denote the layer input corresponding to the calibration data $S$ running through the model. $\widehat{\mathbf{W}}_l$ is the compressed version of $\mathbf{W}_l$. $S$ is generally a subset of LLM pre-training datasets (e.g., WikiText and C4~\citep{RaffelSRLNMZLL20}) for general deployment, or domain-specific datasets for targeted deployment.

%\textbf{Conventional Calibration Data Processing} In typical LLM compression pipelines, the preparation of calibration data $S$ follows a standardized process. The pipeline first loads the calibration datasets and processes them through the model's tokenizer with appropriate error handling mechanisms. A critical preprocessing step involves proper handling of special tokens, particularly ensuring the pad\_token is properly defined, typically defaulting to the eos\_token if undefined. For generating calibration samples, the pipeline concatenates the text data with delimiters and tokenizes it into a continuous sequence of token IDs. Fixed-length segments are then extracted through random sampling within the valid range of the input sequence, ensuring each calibration sample maintains proper context and structure.

